Hyperbolic Multimodal Representation Learning for Biological Taxonomies

Taxonomic classification in biodiversity research involves organizing biological specimens into structured hierarchies based on evidence, which can come from multiple modalities such as images and genetic information. We investigate whether hyperbolic networks can provide a better embedding space for such hierarchical models. Our method embeds multimodal inputs into a shared hyperbolic space using contrastive and a novel stacked entailment-based objective. Experiments on the BIOSCAN-1M dataset show that hyperbolic embedding achieves competitive performance with Euclidean baselines, and outperforms all other models on unseen species classification using DNA barcodes. However, fine-grained classification and open-world generalization remain challenging. Our framework offers a structure-aware foundation for biodiversity modelling, with potential applications to species discovery, ecological monitoring, and conservation efforts.

==> tab/comparison.tex <==
\begin{table*}[htbp]
    \centering
    \footnotesize
    \setlength{\extrarowheight}{2pt}
    \caption{Comparison of MERU, HyCoCLIP and our method (\textit{Biodiversity Hyperbolic}) across key aspects.}
    \label{tab:model_comparison}
    \rowcolors{2}{gray!10}{white}
    \begin{tabularx}{\textwidth}{@{}L L L L@{}}
        \toprule
        \textbf{Aspect} 
            & \textbf{MERU} 
            & \textbf{HyCoCLIP} 
            & \textbf{Our Work} \\
        \midrule
        Modalities 
            & Image + Text 
            & Image + Text + Object Boxes 
            & Image + DNA Barcode + Taxonomic Labels \\

        Use of Hyperbolic Space 
            & Lorentz hyperboloid model 
            & Lorentz model with compositional constraints 
            & Lorentz hyperboloid model \\

        Hierarchy Source 
            & \makecell[l]{Implicit from caption specificity \\ (coarse $\to$ fine)} 
            & \makecell[l]{Implicit composition from \\ part-level object boxes} 
            & \makecell[l]{Explicit taxonomy \\ (Order $\to$ Family $\to$ Genus $\to$ Species)} \\

        Loss Functions 
            & Contrastive + Entailment Loss 
            & Contrastive + Compositional Entailment Loss 
            & Contrastive + Stacked Entailment Loss \\

        Biological Relevance 
            & \xmark\ None 
            & \xmark\ Not domain-specific 
            & Directly applied to biodiversity and species discovery \\

        Classification 
            & \xmark\ No classification setting 
            & \xmark\ No explicit classification 
            & \cmark\ Supports classification of unseen species \\
        \bottomrule
    \end{tabularx}
\end{table*}
